The Soft Anomalous Dimension at four loops in the Regge Limit

The soft anomalous dimension governs the infrared divergences of scattering amplitudes in general kinematics to all orders in perturbation theory. By comparing the recent Regge-limit results for $2\to2$ scattering (through Next-to-Next-to-Leading Logarithms) in full colour to a general form for the soft anomalous dimension at four loops we derive powerful constraints on its kinematic dependence, opening the way for a bootstrap-based determination.

==> mybib.tex <==
 @article{Ma:2020,
   title={A forest formula to subtract infrared singularities in amplitudes for wide-angle scattering},
   volume={2020},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP05(2020)012},
   DOI={10.1007/jhep05(2020)012},
   number={5},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Ma, Yao},
   year={2020},
   month={May}
}
@article{Gardi_2013,
   title={The non-Abelian exponentiation theorem for multiple Wilson lines},
   volume={2013},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP06(2013)088},
   DOI={10.1007/jhep06(2013)088},
   number={6},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Gardi, Einan and Smillie, Jennifer M. and White, Chris D.},
   year={2013},
   month={Jun}
}
@article{Gatheral1983ExponentiationOE,
  title={Exponentiation of eikonal cross sections in nonabelian gauge theories},
  author={Jim Gatheral},
  journal={Physics Letters B},
  year={1983},
  volume={133},
  pages={90-94}
}
@article{Gardi:2013ita,
    author = "Gardi, Einan and Smillie, Jennifer M. and White, Chris D.",
    title = "{The Non-Abelian Exponentiation theorem for multiple Wilson lines}",
    eprint = "1304.7040",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "EDINBURGH-2013-07",
    doi = "10.1007/JHEP06(2013)088",
    journal = "JHEP",
    volume = "06",
    pages = "088",
    year = "2013"
}
@article{Frenkel1984NonabelianEE,
  title={Non-abelian eikonal exponentiation},
  author={J. Frenkel and John Taylor},
  journal={Nuclear Physics},
  year={1984},
  volume={246},
  pages={231-245}
}

@article{Reg3:2021,
     author = "Falcioni, Giulio and Gardi, Einan and Maher,Niamh and Milloy, Calum and Vernazza, Leonardo",
    title = "{Scattering amplitudes in the Regge limit and the soft anomalous dimension through four loops}",
    eprint = "21XX.XXXX",
    archivePrefix = "arXiv",
    year = "2021"
}
@article{Vernazza:2021,
    author = "Vernazza, Leonardo and Falcioni, Giulio and Gardi, Einan and Maher,Niamh and Milloy, Calum",
    title = "{Two-parton scattering in the high-energy limit: climbing two- and three-Reggeon ladders}",
    archivePrefix = "arXiv",
    journal = "PoS",
    volume = "RADCOR2021",
    year = "2021"
}
@inproceedings{Kotikov:2001sc,
    author = "Kotikov, A. V. and Lipatov, L. N.",
    title = "{DGLAP and BFKL evolution equations in the N=4 supersymmetric gauge theory}",
    booktitle = "{35th Annual Winter School on Nuclear and Particle Physics}",
    eprint = "hep-ph/0112346",
    archivePrefix = "arXiv",
    reportNumber = "DESY-02-002",
    month = "12",
    year = "2001"
}

@article{Kotikov:2002ab,
    author = "Kotikov, A. V. and Lipatov, L. N.",
    title = "{DGLAP and BFKL equations in the $N=4$ supersymmetric gauge theory}",
    eprint = "hep-ph/0208220",
    archivePrefix = "arXiv",
    doi = "10.1016/S0550-3213(03)00264-5",
    journal = "Nucl. Phys. B",
    volume = "661",
    pages = "19--61",
    year = "2003",
    note = "[Erratum: Nucl.Phys.B 685, 405--407 (2004)]"
}

@article{Kotikov:2004er,
    author = "Kotikov, A. V. and Lipatov, L. N. and Onishchenko, A. I. and Velizhanin, V. N.",
    title = "{Three loop universal anomalous dimension of the Wilson operators in $N=4$ SUSY Yang-Mills model}",
    eprint = "hep-th/0404092",
    archivePrefix = "arXiv",
    reportNumber = "WSU-HEP-0405",
    doi = "10.1016/j.physletb.2004.05.078",
    journal = "Phys. Lett. B",
    volume = "595",
    pages = "521--529",
    year = "2004",
    note = "[Erratum: Phys.Lett.B 632, 754--756 (2006)]"
}

@article{Kotikov:2007cy,
    author = "Kotikov, A. V. and Lipatov, L. N. and Rej, A. and Staudacher, M. and Velizhanin, V. N.",
    title = "{Dressing and wrapping}",
    eprint = "0704.3586",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "AEI-2007-024",
    doi = "10.1088/1742-5468/2007/10/P10003",
    journal = "J. Stat. Mech.",
    volume = "0710",
    pages = "P10003",
    year = "2007"
}

@article{FormFactors,
      author         = "Moch, S. and Vermaseren, J. A. M. and Vogt, A.",
      title          = "{Three-loop results for quark and gluon form-factors}",
      journal        = "Phys. Lett.",
      volume         = "B625",
      year           = "2005",
      pages          = "245-252",
      doi            = "10.1016/j.physletb.2005.08.067",
      eprint         = "hep-ph/0508055",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "DESY-05-138, SFT-CPP-05-34, NIKHEF-05-013, DCPT-05-88,
                        IPPP-05-44",
      SLACcitation   = "%%CITATION = HEP-PH/0508055;%%"
}

@article{vonManteuffel:2020vjv,
    author = "von Manteuffel, Andreas and Panzer, Erik and Schabinger, Robert M.",
    title = "{Cusp and collinear anomalous dimensions in four-loop QCD from form factors}",
    eprint = "2002.04617",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MSUHEP-20-002",
    doi = "10.1103/PhysRevLett.124.162001",
    journal = "Phys. Rev. Lett.",
    volume = "124",
    number = "16",
    pages = "162001",
    year = "2020"
}
@article{POLYAKOV:1980,
title = {Gauge fields as rings of glue},
journal = {Nuclear Physics B},
volume = {164},
pages = {171-188},
year = {1980},
issn = {0550-3213},
doi = {https://doi.org/10.1016/0550-3213(80)90507-6},
url = {https://www.sciencedirect.com/science/article/pii/0550321380905076},
author = {A.M. Polyakov}}

@article{Berends:1988zn,
title = {Multiple soft gluon radiation in parton processes},
journal = {Nuclear Physics B},
volume = {313},
number = {3},
pages = {595-633},
year = {1989},
issn = {0550-3213},
doi = {https://doi.org/10.1016/0550-3213(89)90398-2},
url = {https://www.sciencedirect.com/science/article/pii/0550321389903982},
author = {F.A. Berends and W.T. Giele}
}
@article{Mangano_1991,
   title={Multi-parton amplitudes in gauge theories},
   volume={200},
   ISSN={0370-1573},
   url={http://dx.doi.org/10.1016/0370-1573(91)90091-Y},
   DOI={10.1016/0370-1573(91)90091-y},
   number={6},
   journal={Physics Reports},
   publisher={Elsevier BV},
   author={Mangano, Michelangelo L. and Parke, Stephen J.},
   year={1991},
   month={Feb},
   pages={301–367}
}
@article{Kosower_1999,
   title={All-order collinear behavior in gauge theories},
   volume={552},
   ISSN={0550-3213},
   url={http://dx.doi.org/10.1016/S0550-3213(99)00251-5},
   DOI={10.1016/s0550-3213(99)00251-5},
   number={1-2},
   journal={Nuclear Physics B},
   publisher={Elsevier BV},
   author={Kosower, David A.},
   year={1999},
   month={Jul},
   pages={319–336}
}
@article{Bern_1995,
   title={Factorization in one-loop gauge theory},
   volume={447},
   ISSN={0550-3213},
   url={http://dx.doi.org/10.1016/0550-3213(95)00226-I},
   DOI={10.1016/0550-3213(95)00226-i},
   number={2-3},
   journal={Nuclear Physics B},
   publisher={Elsevier BV},
   author={Bern, Zvi and Chalmers, Gordon},
   year={1995},
   month={Aug},
   pages={465–518}
}

@article{Henn:2019swt,
    author = "Henn, Johannes M. and Korchemsky, Gregory P. and Mistlberger, Bernhard",
    title = "{The full four-loop cusp anomalous dimension in $\mathcal{N}=4$ super Yang-Mills and QCD}",
    eprint = "1911.10174",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "IPhT-T19/155, MIT-CTP/5160, MPP-2019-233",
    doi = "10.1007/JHEP04(2020)018",
    journal = "JHEP",
    volume = "04",
    pages = "018",
    year = "2020"
}

@article{Falcioni:2020lvv,
    author = "Falcioni, Giulio and Gardi, Einan and Milloy, Calum and Vernazza, Leonardo",
    title = "{Climbing three-Reggeon ladders: four-loop amplitudes in the high-energy limit in full colour}",
    eprint = "2012.00613",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.103.L111501",
    journal = "Phys. Rev. D",
    volume = "103",
    pages = "L111501",
    year = "2021"
}

@article{Naculich:2020clm,
    author = "Naculich, Stephen G.",
    title = "{All-loop-orders relation between Regge limits of $ \mathcal{N} $ = 4 SYM and $ \mathcal{N} $ = 8 supergravity four-point amplitudes}",
    eprint = "2012.00030",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "BOW-PH-169",
    doi = "10.1007/JHEP02(2021)044",
    journal = "JHEP",
    volume = "02",
    pages = "044",
    year = "2021"
}


@article{Dokshitzer:2005ek,
    author = "Dokshitzer, Yu.L. and Marchesini, G.",
    title = "{Hadron collisions and the fifth form-factor}",
    eprint = "hep-ph/0508130",
    archivePrefix = "arXiv",
    reportNumber = "BICOCCA-FT-05-20, LPTHE-05-21",
    doi = "10.1016/j.physletb.2005.10.009",
    journal = "Phys. Lett. B",
    volume = "631",
    pages = "118--125",
    year = "2005"
}

@article{Henn:2016jdu,
    author = "Henn, Johannes M. and Mistlberger, Bernhard",
    title = "{Four-Gluon Scattering at Three Loops, Infrared Structure, and the Regge Limit}",
    eprint = "1608.00850",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-TH-2016-174, MITP-16-084",
    doi = "10.1103/PhysRevLett.117.171601",
    journal = "Phys. Rev. Lett.",
    volume = "117",
    number = "17",
    pages = "171601",
    year = "2016"
}

@article{Gardi:2019pmk,
    author = "Gardi, Einan and Caron-Huot, Simon and Reichel, Joscha and Vernazza, Leonardo",
    title = "{The High-Energy Limit of 2-to-2 Partonic Scattering Amplitudes}",
    eprint = "1912.10883",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.22323/1.375.0050",
    journal = "PoS",
    volume = "RADCOR2019",
    pages = "050",
    year = "2019"
}
@mastersthesis{Mark,
    title    = {Long-Distance Singularities in QCD Scattering Amplitudes},
    school   = {University of Edinburgh},
    author   = {Harley,Mark},
    year     = {2011}
    }
@article{Lipatov:1993yb,
      author         = "Lipatov, L. N.",
      title          = "{Asymptotic behavior of multicolor QCD at high energies
                        in connection with exactly solvable spin models}",
      journal        = "JETP Lett.",
      volume         = "59",
      year           = "1994",
      pages          = "596-599",
      note           = "[Pisma Zh. Eksp. Teor. Fiz.59,571(1994)]",
      eprint         = "hep-th/9311037",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "DFPD-93-TH-70",
      SLACcitation   = "%%CITATION = HEP-TH/9311037;%%"
}


@article{Faddeev:1994zg,
      author         = "Faddeev, L. D. and Korchemsky, G. P.",
      title          = "{High-energy QCD as a completely integrable model}",
      journal        = "Phys. Lett.",
      volume         = "B342",
      year           = "1995",
      pages          = "311-322",
      doi            = "10.1016/0370-2693(94)01363-H",
      eprint         = "hep-th/9404173",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-th",
      reportNumber   = "ITP-SB-94-14",
      SLACcitation   = "%%CITATION = HEP-TH/9404173;%%"
}

@article{DelDuca:2019tur,
    author = "Del Duca, V. and Druc, S. and Drummond, J.M. and Duhr, C. and Dulat, F. and Marzucca, R. and Papathanasiou, G. and Verbeek, B.",
    title = "{All-order amplitudes at any multiplicity in the multi-Regge limit}",
    eprint = "1912.00188",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-19-180, CERN-TH-2019-204, IPPP/19/86, UUITP-48/19, SLAC-PUB-17491",
    doi = "10.1103/PhysRevLett.124.161602",
    journal = "Phys. Rev. Lett.",
    volume = "124",
    number = "16",
    pages = "161602",
    year = "2020"
}

@article{Bartels:2020twc,
    author = "Bartels, Jochen",
    title = "{Analytic structure of the 8-point scattering amplitude in multi-Regge kinematics in $N$=4 SYM : conformal Regge pole and Regge cut contributions}",
    eprint = "2005.08818",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY-20-049",
    month = "5",
    year = "2020"
}

@article{Dixon:2012yy,
    author = "Dixon, Lance J. and Duhr, Claude and Pennington, Jeffrey",
    title = "{Single-valued harmonic polylogarithms and the multi-Regge limit}",
    eprint = "1207.0186",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-15132",
    doi = "10.1007/JHEP10(2012)074",
    journal = "JHEP",
    volume = "10",
    pages = "074",
    year = "2012"
}

@article{Kuraev:1977fs,
      author         = "Kuraev, E. A. and Lipatov, L. N. and Fadin, Victor S.",
      title          = "{The Pomeranchuk Singularity in Nonabelian Gauge
                        Theories}",
      journal        = "Sov. Phys. JETP",
      volume         = "45",
      year           = "1977",
      pages          = "199-204",
      note           = "[Zh. Eksp. Teor. Fiz.72,377(1977)]",
      SLACcitation   = "%%CITATION = SPHJA,45,199;%%"
}

@article{Balitsky:1978ic,
      author         = "Balitsky, I. I. and Lipatov, L. N.",
      title          = "{The Pomeranchuk Singularity in Quantum Chromodynamics}",
      journal        = "Sov. J. Nucl. Phys.",
      volume         = "28",
      year           = "1978",
      pages          = "822-829",
      note           = "[Yad. Fiz.28,1597(1978)]",
      SLACcitation   = "%%CITATION = SJNCA,28,822;%%"
}


@book{Collins:1977jy,
      author         = "Collins, P. D. B.",
      title          = "{An Introduction to Regge Theory and High-Energy
                        Physics}",
      publisher      = "Cambridge Univ. Press",
      address        = "Cambridge, UK",
      year           = "2009",
      url            = "http://www-spires.fnal.gov/spires/find/books/www?cl=QC793.3.R4C695",
      series         = "Cambridge Monographs on Mathematical Physics",
      ISBN           = "9780521110358",
      SLACcitation   = "%%CITATION = INSPIRE-127083;%%"
}

@article{Low:1975sv,
      author         = "Low, F. E.",
      title          = "{A Model of the Bare Pomeron}",
      journal        = "Phys. Rev.",
      volume         = "D12",
      year           = "1975",
      pages          = "163-173",
      doi            = "10.1103/PhysRevD.12.163",
      reportNumber   = "MIT-CTP-438",
      SLACcitation   = "%%CITATION = PHRVA,D12,163;%%"
}
  
@article{Nussinov:1975mw,
      author         = "Nussinov, S.",
      title          = "{Colored Quark Version of Some Hadronic Puzzles}",
      journal        = "Phys. Rev. Lett.",
      volume         = "34",
      year           = "1975",
      pages          = "1286-1289",
      doi            = "10.1103/PhysRevLett.34.1286",
      reportNumber   = "TAUP-462-75",
      SLACcitation   = "%%CITATION = PRLTA,34,1286;%%"
}
 
@article{Gunion:1976iy,
      author         = "Gunion, J. F. and Soper, Davison E.",
      title          = "{Quark Counting and Hadron Size Effects for Total
                        Cross-Sections}",
      journal        = "Phys. Rev.",
      volume         = "D15",
      year           = "1977",
      pages          = "2617-2621",
      doi            = "10.1103/PhysRevD.15.2617",
      reportNumber   = "PRINT-76-0955 (UC,DAVIS)",
      SLACcitation   = "%%CITATION = PHRVA,D15,2617;%%"
}

@article{Korchemskaya:1994qp,
      author         = "Korchemskaya, I. A. and Korchemsky, G. P.",
      title          = "{High-energy scattering in QCD and cross singularities of
                        Wilson loops}",
      journal        = "Nucl. Phys.",
      volume         = "B437",
      year           = "1995",
      pages          = "127-162",
      doi            = "10.1016/0550-3213(94)00553-Q",
      eprint         = "hep-ph/9409446",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "ITP-SB-94-42",
      SLACcitation   = "%%CITATION = HEP-PH/9409446;%%"
}

@article{Korchemsky:1991zp,
    author = "Korchemsky, G. P. and Radyushkin, A. V.",
    title = "{Infrared factorization, Wilson lines and the heavy quark limit}",
    eprint = "hep-ph/9203222",
    archivePrefix = "arXiv",
    reportNumber = "CPT-91-P-2629",
    doi = "10.1016/0370-2693(92)90405-S",
    journal = "Phys. Lett. B",
    volume = "279",
    pages = "359--366",
    year = "1992"
}


@article{Korchemskaya:1996je,
      author         = "Korchemskaya, I. A. and Korchemsky, G. P.",
      title          = "{Evolution equation for gluon Regge trajectory}",
      journal        = "Phys. Lett.",
      volume         = "B387",
      year           = "1996",
      pages          = "346-354",
      doi            = "10.1016/0370-2693(96)01016-7",
      eprint         = "hep-ph/9607229",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "LPTHE-ORSAY-96-53",
      SLACcitation   = "%%CITATION = HEP-PH/9607229;%%"
}

@article{Balitsky:1995ub,
      author         = "Balitsky, I.",
      title          = "{Operator expansion for high-energy scattering}",
      journal        = "Nucl. Phys.",
      volume         = "B463",
      year           = "1996",
      pages          = "99-160",
      doi            = "10.1016/0550-3213(95)00638-9",
      eprint         = "hep-ph/9509348",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "MIT-CTP-2470",
      SLACcitation   = "%%CITATION = HEP-PH/9509348;%%"
}

@article{Kovchegov:1999yj,
      author         = "Kovchegov, Yuri V.",
      title          = "{Small x F(2) structure function of a nucleus including
                        multiple pomeron exchanges}",
      journal        = "Phys. Rev.",
      volume         = "D60",
      year           = "1999",
      pages          = "034008",
      doi            = "10.1103/PhysRevD.60.034008",
      eprint         = "hep-ph/9901281",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "NUC-MN-99-1-T, TPI-MINN-99-05",
      SLACcitation   = "%%CITATION = HEP-PH/9901281;%%"
}

@article{JalilianMarian:1996xn,
      author         = "Jalilian-Marian, Jamal and Kovner, Alex and McLerran,
                        Larry D. and Weigert, Heribert",
      title          = "{The Intrinsic glue distribution at very small x}",
      journal        = "Phys. Rev.",
      volume         = "D55",
      year           = "1997",
      pages          = "5414-5428",
      doi            = "10.1103/PhysRevD.55.5414",
      eprint         = "hep-ph/9606337",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TPI-MINN-96-1429, NUC-MINN-96-10-T, TPI-MINN-96-08",
      SLACcitation   = "%%CITATION = HEP-PH/9606337;%%"
}

@article{JalilianMarian:1997gr,
      author         = "Jalilian-Marian, Jamal and Kovner, Alex and Leonidov,
                        Andrei and Weigert, Heribert",
      title          = "{The Wilson renormalization group for low x physics:
                        Towards the high density regime}",
      journal        = "Phys. Rev.",
      volume         = "D59",
      year           = "1998",
      pages          = "014014",
      doi            = "10.1103/PhysRevD.59.014014",
      eprint         = "hep-ph/9706377",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "TPI-MINN-97-20-T, NUC-MINN-97-6-T, HEP-MINN-97-1546,
                        CAVENDISH-HEP-97-09",
      SLACcitation   = "%%CITATION = HEP-PH/9706377;%%"
}

@article{Gribov:1973iv,
    author = "Gribov, V. N. and Anselm, A. A.",
    title = "{Weak interactions at high-energies and complex angular momenta}",
    doi = "10.1016/0550-3213(73)90362-3",
    journal = "Nucl. Phys. B",
    volume = "61",
    pages = "253--273",
    year = "1973"
}

@BOOK{Analytic_S-Matrix,
       author = {{Eden}, R.~J. and {Landshoff}, P.~V. and {Olive}, D.~I. and {Polkinghorne}, J.~C.},
        title = "{The Analytic S-Matrix}",
         year = 2002,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002asm..book.....E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
  
@article{Veneziano:1968yb,
    author = "Veneziano, G.",
    title = "{Construction of a crossing - symmetric, Regge behaved amplitude for linearly rising trajectories}",
    doi = "10.1007/BF02824451",
    journal = "Nuovo Cim. A",
    volume = "57",
    pages = "190--197",
    year = "1968"
}  
  
@article{Iancu:2001ad,
      author         = "Iancu, Edmond and Leonidov, Andrei and McLerran, Larry
                        D.",
      title          = "{The Renormalization group equation for the color glass
                        condensate}",
      journal        = "Phys. Lett.",
      volume         = "B510",
      year           = "2001",
      pages          = "133-144",
      doi            = "10.1016/S0370-2693(01)00524-X",
      eprint         = "hep-ph/0102009",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "BNL-NT-01-3",
      SLACcitation   = "%%CITATION = HEP-PH/0102009;%%"
}


%%%%%%%

@article{Dixon:2014voa,
    author = "Dixon, Lance J. and Drummond, James M. and Duhr, Claude and Pennington, Jeffrey",
    title = "{The four-loop remainder function and multi-Regge behavior at NNLLA in planar N = 4 super-Yang-Mills theory}",
    eprint = "1402.3300",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-15902, CERN-PH-TH-2014-027, IPPP-14-09, DCPT-14-18, LAPTH-010-14",
    doi = "10.1007/JHEP06(2014)116",
    journal = "JHEP",
    volume = "06",
    pages = "116",
    year = "2014"
}

@article{Magnus_Wilhelm,
author = {Magnus, Wilhelm},
title = {On the exponential solution of differential equations for a linear operator},
journal = {Communications on Pure and Applied Mathematics},
volume = {7},
number = {4},
pages = {649-673},
doi = {https://doi.org/10.1002/cpa.3160070404},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/cpa.3160070404},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/cpa.3160070404},
year = {1954}
}

@article{Caron-Huot:2017fxr,
      author         = "Caron-Huot, Simon and Gardi, Einan and Vernazza,
                        Leonardo",
      title          = "{Two-parton scattering in the high-energy limit}",
      journal        = "JHEP",
      volume         = "06",
      year           = "2017",
      pages          = "016",
      doi            = "10.1007/JHEP06(2017)016",
      eprint         = "1701.05241",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "EDINBURGH-2017-01",
      SLACcitation   = "%%CITATION = ARXIV:1701.05241;%%"
}
@article{DelDuca:2011ae,
    author = "Del Duca, Vittorio and Duhr, Claude and Gardi, Einan and Magnea, Lorenzo and White, Chris D.",
    title = "{The Infrared structure of gauge theory amplitudes in the high-energy limit}",
    eprint = "1109.3581",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPPP-11-48, DCPT-11-96, EDINBURGH-2011-22, DFTT-24-2011",
    doi = "10.1007/JHEP12(2011)021",
    journal = "JHEP",
    volume = "12",
    pages = "021",
    year = "2011"
}

@article{Caron-Huot:2016owq,
    author = "Caron-Huot, Simon and Dixon, Lance J. and McLeod, Andrew and von Hippel, Matt",
    title = "{Bootstrapping a Five-Loop Amplitude Using Steinmann Relations}",
    eprint = "1609.00669",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-16811",
    doi = "10.1103/PhysRevLett.117.241601",
    journal = "Phys. Rev. Lett.",
    volume = "117",
    number = "24",
    pages = "241601",
    year = "2016"
}

@article{Caron-Huot:2019vjl,
    author = "Caron-Huot, Simon and Dixon, Lance J. and Dulat, Falko and von Hippel, Matt and McLeod, Andrew J. and Papathanasiou, Georgios",
    title = "{Six-Gluon amplitudes in planar $ \mathcal{N} $ = 4 super-Yang-Mills theory at six and seven loops}",
    eprint = "1903.10890",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DESY 19-042, HU-EP-19/04, DESY-19-042, HU-EP-19-04, SLAC-PUB-17413",
    doi = "10.1007/JHEP08(2019)016",
    journal = "JHEP",
    volume = "08",
    pages = "016",
    year = "2019"
}

@article{Caron-Huot:2017zfo,
    author = "Caron-Huot, Simon and Gardi, Einan and Reichel, Joscha and Vernazza, Leonardo",
    archivePrefix = "arXiv",
    doi = "10.1007/JHEP03(2018)098",
    eprint = "1711.04850",
    journal = "JHEP",
    pages = "098",
    primaryClass = "hep-ph",
    reportNumber = "EDINBURGH-2017-24, NIKHEF-2017-060",
    title = "{Infrared singularities of QCD scattering amplitudes in the Regge limit to all orders}",
    volume = "03",
    year = "2018"
}


@article{Caron-Huot:2020grv,
    author = "Caron-Huot, Simon and Gardi, Einan and Reichel, Joscha and Vernazza, Leonardo",
    title = "{Two-parton scattering amplitudes in the Regge limit to high loop orders}",
    eprint = "2006.01267",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP08(2020)116",
    journal = "JHEP",
    volume = "08",
    pages = "116",
    year = "2020"
}
@article{upcoming,
author = "Falcioni, Giulio and Gardi, Einan and Milloy, Calum and Vernazza, Leonardo",
journal = "Scattering amplitudes in the Regge limit and the soft anomalous dimension through four loops, in preparation.",
title = "{Upcoming}",
year = "2021"
}

@article{Almelid:2017qju,
    author = "Almelid, \O{}yvind and Duhr, Claude and Gardi, Einan and McLeod, Andrew and White, Chris D.",
    title = "{Bootstrapping the QCD soft anomalous dimension}",
    eprint = "1706.10162",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "EDINBURGH-2017-13, CERN-TH-2017-138, CP3-17-20, SLAC-PUB-17089, QMUL-PH-17-10",
    doi = "10.1007/JHEP09(2017)073",
    journal = "JHEP",
    volume = "09",
    pages = "073",
    year = "2017"
}

@article{Almelid:2015jia,
    author = "Almelid, \O{}yvind and Duhr, Claude and Gardi, Einan",
    title = "{Three-loop corrections to the soft anomalous dimension in multileg scattering}",
    eprint = "1507.00047",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2015-148, CP3-15-18, EDINBURGH-2015-08, LPN15-026",
    doi = "10.1103/PhysRevLett.117.172002",
    journal = "Phys. Rev. Lett.",
    volume = "117",
    number = "17",
    pages = "172002",
    year = "2016"
}
@article{Gardi:2009qi,
    author = "Gardi, Einan and Magnea, Lorenzo",
    title = "{Factorization constraints for soft anomalous dimensions in QCD scattering amplitudes}",
    eprint = "0901.1091",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "EDINBURGH-2008-35, DFTT-29-2008",
    doi = "10.1088/1126-6708/2009/03/079",
    journal = "JHEP",
    volume = "03",
    pages = "079",
    year = "2009"
}
@article{Becher:2009cu,
    author = "Becher, Thomas and Neubert, Matthias",
    title = "{Infrared singularities of scattering amplitudes in perturbative QCD}",
    eprint = "0901.0722",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-09-002-T, MZ-TH-09-01",
    doi = "10.1103/PhysRevLett.102.162001",
    journal = "Phys. Rev. Lett.",
    volume = "102",
    pages = "162001",
    year = "2009",
    note = "[Erratum: Phys.Rev.Lett. 111, 199905 (2013)]"
}



@article{Caron-Huot:2013fea,
    author = "Caron-Huot, Simon",
    title = "{When does the gluon reggeize?}",
    eprint = "1309.6521",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP05(2015)093",
    journal = "JHEP",
    volume = "05",
    pages = "093",
    year = "2015"
}
@article{Becher:2019avh,
    author = "Becher, Thomas and Neubert, Matthias",
    title = "{Infrared singularities of scattering amplitudes and N$^{3}$LL resummation for $n$-jet processes}",
    eprint = "1908.11379",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MZ-TH/19-056",
    doi = "10.1007/JHEP01(2020)025",
    journal = "JHEP",
    volume = "01",
    pages = "025",
    year = "2020"
}

@article{Boels:2017ftb,
    author = "Boels, Rutger H. and Huber, Tobias and Yang, Gang",
    title = "{The Sudakov form factor at four loops in maximal super Yang-Mills theory}",
    eprint = "1711.08449",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SI-HEP-2017-26",
    doi = "10.1007/JHEP01(2018)153",
    journal = "JHEP",
    volume = "01",
    pages = "153",
    year = "2018"
}



@article{Moch:2017uml,
    author = "Moch, S. and Ruijl, B. and Ueda, T. and Vermaseren, J. A. M. and Vogt, A.",
    title = "{Four-Loop Non-Singlet Splitting Functions in the Planar Limit and Beyond}",
    eprint = "1707.08315",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-17-106, NIKHEF-2017-034, LTH-1139",
    doi = "10.1007/JHEP10(2017)041",
    journal = "JHEP",
    volume = "10",
    pages = "041",
    year = "2017"
}

@article{Grozin:2017css,
    author = "Grozin, Andrey and Henn, Johannes and Stahlhofen, Maximilian",
    title = "{On the Casimir scaling violation in the cusp anomalous dimension at small angle}",
    eprint = "1708.01221",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MITP-17-050",
    doi = "10.1007/JHEP10(2017)052",
    journal = "JHEP",
    volume = "10",
    pages = "052",
    year = "2017"
}

@article{Boels:2017skl,
    author = "Boels, Rutger H. and Huber, Tobias and Yang, Gang",
    title = "{Four-Loop Nonplanar Cusp Anomalous Dimension in N=4 Supersymmetric Yang-Mills Theory}",
    eprint = "1705.03444",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SI-HEP-2017-10",
    doi = "10.1103/PhysRevLett.119.201601",
    journal = "Phys. Rev. Lett.",
    volume = "119",
    number = "20",
    pages = "201601",
    year = "2017"
}


@article{Korchemsky:1987wg,
    author = "Korchemsky, G.P. and Radyushkin, A.V.",
    title = "{Renormalization of the Wilson Loops Beyond the Leading Order}",
    doi = "10.1016/0550-3213(87)90277-X",
    journal = "Nucl. Phys. B",
    volume = "283",
    pages = "342--364",
    year = "1987"
}

@article{Lee:2013mka,
    author = "Lee, Roman N.",
    editor = "Wang, Jianxiong",
    title = "{LiteRed 1.4: a powerful tool for reduction of multiloop integrals}",
    eprint = "1310.1145",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1742-6596/523/1/012059",
    journal = "J. Phys. Conf. Ser.",
    volume = "523",
    pages = "012059",
    year = "2014"
}

@article{Ruijl:2017cxj,
    author = "Ruijl, B. and Ueda, T. and Vermaseren, J.A.M.",
    title = "{Forcer, a FORM program for the parametric reduction of four-loop massless propagator diagrams}",
    eprint = "1704.06650",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "NIKHEF-2017-019",
    doi = "10.1016/j.cpc.2020.107198",
    journal = "Comput. Phys. Commun.",
    volume = "253",
    pages = "107198",
    year = "2020"
}
@article{Bern:2005iz,
    author = "Bern, Zvi and Dixon, Lance J. and Smirnov, Vladimir A.",
    title = "{Iteration of planar amplitudes in maximally supersymmetric Yang-Mills theory at three loops and beyond}",
    eprint = "hep-th/0505205",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-11210, UCLA-05-TEP-14",
    doi = "10.1103/PhysRevD.72.085001",
    journal = "Phys. Rev. D",
    volume = "72",
    pages = "085001",
    year = "2005"
}

@article{Catani:1996jh,
    author = "Catani, S. and Seymour, M. H.",
    title = "{The Dipole formalism for the calculation of QCD jet cross-sections at next-to-leading order}",
    eprint = "hep-ph/9602277",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-96-28",
    doi = "10.1016/0370-2693(96)00425-X",
    journal = "Phys. Lett. B",
    volume = "378",
    pages = "287--301",
    year = "1996"
}

@article{Catani:1996vz,
    author = "Catani, S. and Seymour, M. H.",
    title = "{A General algorithm for calculating jet cross-sections in NLO QCD}",
    eprint = "hep-ph/9605323",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-96-029, CERN-TH-96-29",
    doi = "10.1016/S0550-3213(96)00589-5",
    journal = "Nucl. Phys. B",
    volume = "485",
    pages = "291--419",
    year = "1997",
    note = "[Erratum: Nucl.Phys.B 510, 503--504 (1998)]"
}

@article{Catani:1998bh,
    author = "Catani, Stefano",
    title = "{The Singular behavior of QCD amplitudes at two loop order}",
    eprint = "hep-ph/9802439",
    archivePrefix = "arXiv",
    reportNumber = "CERN-TH-98-42, LPTHE-ORSAY-97-57",
    doi = "10.1016/S0370-2693(98)00332-3",
    journal = "Phys. Lett. B",
    volume = "427",
    pages = "161--171",
    year = "1998"
}
@article{Sterman:2002qn,
    author = "Sterman, George F. and Tejeda-Yeomans, Maria E.",
    title = "{Multiloop amplitudes and resummation}",
    eprint = "hep-ph/0210130",
    archivePrefix = "arXiv",
    reportNumber = "YITP-SB-02-56",
    doi = "10.1016/S0370-2693(02)03100-3",
    journal = "Phys. Lett. B",
    volume = "552",
    pages = "48--56",
    year = "2003"
}
@article{Aybat:2006wq,
    author = "Aybat, S.Mert and Dixon, Lance J. and Sterman, George F.",
    title = "{The Two-loop anomalous dimension matrix for soft gluon exchange}",
    eprint = "hep-ph/0606254",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-11907, YITP-SB-06-25",
    doi = "10.1103/PhysRevLett.97.072001",
    journal = "Phys. Rev. Lett.",
    volume = "97",
    pages = "072001",
    year = "2006"
}
@article{Aybat:2006mz,
    author = "Aybat, S.Mert and Dixon, Lance J. and Sterman, George F.",
    title = "{The Two-loop soft anomalous dimension matrix and resummation at next-to-next-to leading pole}",
    eprint = "hep-ph/0607309",
    archivePrefix = "arXiv",
    reportNumber = "YITP-SB-06-28, SLAC-PUB-11969",
    doi = "10.1103/PhysRevD.74.074004",
    journal = "Phys. Rev. D",
    volume = "74",
    pages = "074004",
    year = "2006"
}
@article{Gardi:2009zv,
    author = "Gardi, Einan and Magnea, Lorenzo",
    editor = "Greco, Mario",
    title = "{Infrared singularities in QCD amplitudes}",
    eprint = "0908.3273",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "EDINBURGH-2009-09",
    doi = "10.1393/ncc/i2010-10528-x",
    journal = "Frascati Phys. Ser.",
    volume = "50",
    pages = "137--157",
    year = "2010"
}

@article{Lipatov:1976zz,
    author = "Lipatov, L.N.",
    title = "{Reggeization of the Vector Meson and the Vacuum Singularity in Nonabelian Gauge Theories}",
    journal = "Sov. J. Nucl. Phys.",
    volume = "23",
    pages = "338--345",
    year = "1976"
}

@article{Kuraev:1976ge,
    author = "Kuraev, E. A. and Lipatov, L. N. and Fadin, Victor S.",
    title = "{Multi - Reggeon Processes in the Yang-Mills Theory}",
    journal = "Sov. Phys. JETP",
    volume = "44",
    pages = "443--450",
    year = "1976"
}

@article{Moch:2004pa,
    author = "Moch, S. and Vermaseren, J.A.M. and Vogt, A.",
    title = "{The Three loop splitting functions in QCD: The Nonsinglet case}",
    eprint = "hep-ph/0403192",
    archivePrefix = "arXiv",
    reportNumber = "DESY-04-047, SFB-CPP-04-09, NIKHEF-04-001",
    doi = "10.1016/j.nuclphysb.2004.03.030",
    journal = "Nucl. Phys. B",
    volume = "688",
    pages = "101--134",
    year = "2004"
}

@article{Dixon:2008gr,
    author = "Dixon, Lance J. and Magnea, Lorenzo and Sterman, George F.",
    title = "{Universal structure of subleading infrared poles in gauge theory amplitudes}",
    eprint = "0805.3515",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "YITP-SB-08-16, DFTT-06-2008, SLAC-PUB-13141",
    doi = "10.1088/1126-6708/2008/08/022",
    journal = "JHEP",
    volume = "08",
    pages = "022",
    year = "2008"
}

@article{Fadin:2006bj,
    author = "Fadin, V.S. and Fiore, R. and Kozlov, M.G. and Reznichenko, A.V.",
    title = "{Proof of the multi-Regge form of QCD amplitudes with gluon exchanges in the NLA}",
    eprint = "hep-ph/0602006",
    archivePrefix = "arXiv",
    doi = "10.1016/j.physletb.2006.03.031",
    journal = "Phys. Lett. B",
    volume = "639",
    pages = "74--81",
    year = "2006"
}

@article{Fadin:2015zea,
    author = "Fadin, V.S. and Kozlov, M.G. and Reznichenko, A.V.",
    title = "{Gluon Reggeization in Yang-Mills Theories}",
    eprint = "1507.00823",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "Budker-INP-2014-19",
    doi = "10.1103/PhysRevD.92.085044",
    journal = "Phys. Rev. D",
    volume = "92",
    number = "8",
    pages = "085044",
    year = "2015"
}

@article{Fadin:1995xg,
    author = "Fadin, Victor S. and Kotsky, M.I. and Fiore, R.",
    title = "{Gluon Reggeization in QCD in the next-to-leading order}",
    doi = "10.1016/0370-2693(95)01016-J",
    journal = "Phys. Lett. B",
    volume = "359",
    pages = "181--188",
    year = "1995"
}

@article{Fadin:1996tb,
    author = "Fadin, Victor S. and Fiore, R. and Kotsky, M.I.",
    title = "{Gluon Regge trajectory in the two loop approximation}",
    eprint = "hep-ph/9605357",
    archivePrefix = "arXiv",
    reportNumber = "BUDKER-INP-1996-35, CS-TH-3-96",
    doi = "10.1016/0370-2693(96)01054-4",
    journal = "Phys. Lett. B",
    volume = "387",
    pages = "593--602",
    year = "1996"
}

@article{Fadin:1995km,
    author = "Fadin, Victor S. and Fiore, R. and Quartarolo, A.",
    title = "{Reggeization of quark quark scattering amplitude in QCD}",
    eprint = "hep-ph/9506432",
    archivePrefix = "arXiv",
    reportNumber = "BUDKER-INP-1995-49, CS-TH-12-95",
    doi = "10.1103/PhysRevD.53.2729",
    journal = "Phys. Rev. D",
    volume = "53",
    pages = "2729--2741",
    year = "1996"
}

@article{Blumlein:1998ib,
    author = "Blumlein, J. and Ravindran, V. and van Neerven, W.L.",
    title = "{On the gluon Regge trajectory in O alpha-s**2}",
    eprint = "hep-ph/9806357",
    archivePrefix = "arXiv",
    reportNumber = "DESY-98-067",
    doi = "10.1103/PhysRevD.58.091502",
    journal = "Phys. Rev. D",
    volume = "58",
    pages = "091502",
    year = "1998"
}

@article{Fadin:2017nka,
    author = "Fadin, V.S. and Lipatov, L.N.",
    title = "{Reggeon cuts in QCD amplitudes with negative signature}",
    eprint = "1712.09805",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "BUDKER-INP-2017-15",
    doi = "10.1140/epjc/s10052-018-5910-1",
    journal = "Eur. Phys. J. C",
    volume = "78",
    number = "6",
    pages = "439",
    year = "2018"
}

@article{Fadin:2016wso,
    author = "Fadin, V.S.",
    editor = "Capua, Marcella and Fiore, Roberto and Papa, Alessandro and Rossi, Marco and Solano, Ada and Tassi, Enrico",
    title = "{Particularities of the NNLLA BFKL}",
    eprint = "1612.04481",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1063/1.4977159",
    journal = "AIP Conf. Proc.",
    volume = "1819",
    number = "1",
    pages = "060003",
    year = "2017"
}

@article{DelDuca:2001gu,
    author = "Del Duca, Vittorio and Glover, E.W.Nigel",
    title = "{The High-energy limit of QCD at two loops}",
    eprint = "hep-ph/0109028",
    archivePrefix = "arXiv",
    reportNumber = "DCPT-01-66, IPPP-01-33, DFTT-25-2001",
    doi = "10.1088/1126-6708/2001/10/035",
    journal = "JHEP",
    volume = "10",
    pages = "035",
    year = "2001"
}

@article{Korchemsky:1985xj,
    author = "Korchemsky, G. P. and Radyushkin, A. V.",
    title = "{Loop Space Formalism and Renormalization Group for the Infrared Asymptotics of {QCD}}",
    reportNumber = "JINR-P2-85-716",
    doi = "10.1016/0370-2693(86)91439-5",
    journal = "Phys. Lett. B",
    volume = "171",
    pages = "459--467",
    year = "1986"
}

@article{Gehrmann:2010ue,
    author = "Gehrmann, T. and Glover, E. W. N. and Huber, T. and Ikizlerli, N. and Studerus, C.",
    title = "{Calculation of the quark and gluon form factors to three loops in QCD}",
    eprint = "1004.3653",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "ZU-TH-07-10, IPPP-10-26, SI-HEP-2010-09, ZU--TH-07-10",
    doi = "10.1007/JHEP06(2010)094",
    journal = "JHEP",
    volume = "06",
    pages = "094",
    year = "2010"
}

@article{DelDuca:2014cya,
    author = "Del Duca, Vittorio and Falcioni, Giulio and Magnea, Lorenzo and Vernazza, Leonardo",
    title = "{Analyzing high-energy factorization beyond next-to-leading logarithmic accuracy}",
    eprint = "1409.8330",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP02(2015)029",
    journal = "JHEP",
    volume = "02",
    pages = "029",
    year = "2015"
}

@article{DelDuca:2013dsa,
    author = "Del Duca, Vittorio and Falcioni, Giulio and Magnea, Lorenzo and Vernazza, Leonardo",
    title = "{Beyond Reggeization for two- and three-loop QCD amplitudes}",
    eprint = "1312.5098",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.22323/1.197.0046",
    journal = "PoS",
    volume = "RADCOR2013",
    pages = "046",
    year = "2013"
}

@article{DelDuca:2013ara,
    author = "Del Duca, Vittorio and Falcioni, Giulio and Magnea, Lorenzo and Vernazza, Leonardo",
    title = "{High-energy QCD amplitudes at two loops and beyond}",
    eprint = "1311.0304",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "LPN13-086",
    doi = "10.1016/j.physletb.2014.03.033",
    journal = "Phys. Lett. B",
    volume = "732",
    pages = "233--240",
    year = "2014"
}

@article{Balitsky:2001mr,
    author = "Balitsky, I.I. and Belitsky, Andrei V.",
    title = "{Nonlinear evolution in high density QCD}",
    eprint = "hep-ph/0110158",
    archivePrefix = "arXiv",
    reportNumber = "DOE-ER-40762-008, UMD-PP-02-010, YITP-SB-01-44, JLAB-THY-01-27",
    doi = "10.1016/S0550-3213(02)00149-9",
    journal = "Nucl. Phys. B",
    volume = "629",
    pages = "290--322",
    year = "2002"
}

@article{Balitsky:2008zza,
    author = "Balitsky, Ian and Chirilli, Giovanni A.",
    title = "{Next-to-leading order evolution of color dipoles}",
    eprint = "0710.4330",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "JLAB-THY-07-741",
    doi = "10.1103/PhysRevD.77.014019",
    journal = "Phys. Rev. D",
    volume = "77",
    pages = "014019",
    year = "2008"
}

@article{Gardi:2006rp,
    author = "Gardi, Einan and Kuokkanen, Janne and Rummukainen, Kari and Weigert, Heribert",
    title = "{Running coupling and power corrections in nonlinear evolution at the high-energy limit}",
    eprint = "hep-ph/0609087",
    archivePrefix = "arXiv",
    reportNumber = "CERN-PH-TH-2006-170, CAVENDISH-HEP-06-21",
    doi = "10.1016/j.nuclphysa.2006.12.004",
    journal = "Nucl. Phys. A",
    volume = "784",
    pages = "282--340",
    year = "2007"
}

@article{Balitsky:2013fea,
    author = "Balitsky, Ian and Chirilli, Giovanni A.",
    title = "{Rapidity evolution of Wilson lines at the next-to-leading order}",
    eprint = "1309.7644",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "JLAB-THY-13-1806",
    doi = "10.1103/PhysRevD.88.111501",
    journal = "Phys. Rev. D",
    volume = "88",
    pages = "111501",
    year = "2013"
}

@article{Kovner:2013ona,
    author = "Kovner, Alex and Lublinsky, Michael and Mulian, Yair",
    title = "{Jalilian-Marian, Iancu, McLerran, Weigert, Leonidov, Kovner evolution at next to leading order}",
    eprint = "1310.0378",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.89.061704",
    journal = "Phys. Rev. D",
    volume = "89",
    number = "6",
    pages = "061704",
    year = "2014"
}

@article{Drummond:2007aua,
    author = "Drummond, J.M. and Korchemsky, G.P. and Sokatchev, E.",
    title = "{Conformal properties of four-gluon planar amplitudes and Wilson loops}",
    eprint = "0707.0243",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1016/j.nuclphysb.2007.11.041",
    journal = "Nucl. Phys. B",
    volume = "795",
    pages = "385--408",
    year = "2008"
}

@article{Anastasiou:2003kj,
    author = "Anastasiou, C. and Bern, Z. and Dixon, Lance J. and Kosower, D.A.",
    title = "{Planar amplitudes in maximally supersymmetric Yang-Mills theory}",
    eprint = "hep-th/0309040",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-10157, UCLA-03-TEP-23, SACLAY-SPHT-T03-128",
    doi = "10.1103/PhysRevLett.91.251602",
    journal = "Phys. Rev. Lett.",
    volume = "91",
    pages = "251602",
    year = "2003"
}


@article{vanRitbergen:1998pn,
    author = "van Ritbergen, T. and Schellekens, A.N. and Vermaseren, J.A.M.",
    title = "{Group theory factors for Feynman diagrams}",
    eprint = "hep-ph/9802376",
    archivePrefix = "arXiv",
    reportNumber = "UM-TH-98-01, NIKHEF-98-004",
    doi = "10.1142/S0217751X99000038",
    journal = "Int. J. Mod. Phys. A",
    volume = "14",
    pages = "41--96",
    year = "1999"
}

@article{Sjodahl:2012nk,
    author = {Sj\"odahl, Malin},
    title = "{ColorMath - A package for color summed calculations in SU(Nc)}",
    eprint = "1211.2099",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "LU-TP-12-40, MCNET-13-04",
    doi = "10.1140/epjc/s10052-013-2310-4",
    journal = "Eur. Phys. J. C",
    volume = "73",
    number = "2",
    pages = "2310",
    year = "2013"
}

@book{Cvitanovic:2008zz,
    author = "Cvitanovic, Predrag",
    title = "{Group theory: Birdtracks, Lie's and exceptional groups}",
    year = "2008",
    publisher = "Princeton University Press"
}

@article{Falcioni:2019nxk,
    author = "Falcioni, Giulio and Gardi, Einan and Milloy, Calum",
    title = "{Relating amplitude and PDF factorisation through Wilson-line geometries}",
    eprint = "1909.00697",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP11(2019)100",
    journal = "JHEP",
    volume = "11",
    pages = "100",
    year = "2019"
}
@article{Gardi_2013,
   title={The non-Abelian exponentiation theorem for multiple Wilson lines},
   volume={2013},
   ISSN={1029-8479},
   url={http://dx.doi.org/10.1007/JHEP06(2013)088},
   DOI={10.1007/jhep06(2013)088},
   number={6},
   journal={Journal of High Energy Physics},
   publisher={Springer Science and Business Media LLC},
   author={Gardi, Einan and Smillie, Jennifer M. and White, Chris D.},
   year={2013},
   month={Jun}
}
@misc{vladimirov2017structure,
      title={Structure of rapidity divergences in soft factors}, 
      author={Alexey Vladimirov},
      year={2017},
      eprint={1707.07606},
      archivePrefix={arXiv},
      primaryClass={hep-ph}
}

@article{Vladimirov:2017ksc,
    author = "Vladimirov, Alexey",
    title = "{Structure of rapidity divergences in multi-parton scattering soft factors}",
    eprint = "1707.07606",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP04(2018)045",
    journal = "JHEP",
    volume = "04",
    pages = "045",
    year = "2018"
}



@article{Derkachov:2002wz,
    author = "Derkachov, Sergey E. and Korchemsky, G. P. and Kotanski, J. and Manashov, A. N.",
    title = "{Noncompact Heisenberg spin magnets from high-energy QCD. 2. Quantization conditions and energy spectrum}",
    eprint = "hep-th/0204124",
    archivePrefix = "arXiv",
    reportNumber = "LPT-ORSAY-02-30, TPJU-08-2002, UB-ECM-PF-02-07",
    doi = "10.1016/S0550-3213(02)00842-8",
    journal = "Nucl. Phys. B",
    volume = "645",
    pages = "237--297",
    year = "2002"
}

@article{Derkachov:2001yn,
    author = "Derkachov, Sergey E. and Korchemsky, G. P. and Manashov, A. N.",
    title = "{Noncompact Heisenberg spin magnets from high-energy QCD: 1. Baxter Q operator and separation of variables}",
    eprint = "hep-th/0107193",
    archivePrefix = "arXiv",
    reportNumber = "LPT-ORSAY-01-75, UB-ECM-PF-01-05",
    doi = "10.1016/S0550-3213(01)00457-6",
    journal = "Nucl. Phys. B",
    volume = "617",
    pages = "375--440",
    year = "2001"
}

@article{Kazakov:1984bw,
    author = "Kazakov, D. I.",
    title = "{ANALYTICAL METHODS FOR MULTILOOP CALCULATIONS: TWO LECTURES ON THE METHOD OF UNIQUENESS}",
    reportNumber = "JINR-E2-84-410",
    month = "6",
    year = "1984"
}

@article{Tkachov:1981wb,
    author = "Tkachov, F. V.",
    title = "{A Theorem on Analytical Calculability of Four Loop Renormalization Group Functions}",
    doi = "10.1016/0370-2693(81)90288-4",
    journal = "Phys. Lett. B",
    volume = "100",
    pages = "65--68",
    year = "1981"
}

@article{Tarasov:1996br,
    author = "Tarasov, O. V.",
    title = "{Connection between Feynman integrals having different values of the space-time dimension}",
    eprint = "hep-th/9606018",
    archivePrefix = "arXiv",
    reportNumber = "DESY-96-068, JINR-E2-96-62",
    doi = "10.1103/PhysRevD.54.6479",
    journal = "Phys. Rev. D",
    volume = "54",
    pages = "6479--6490",
    year = "1996"
}

@article{Borowka:2017idc,
    author = "Borowka, S. and Heinrich, G. and Jahn, S. and Jones, S. P. and Kerner, M. and Schlenk, J. and Zirke, T.",
    title = "{pySecDec: a toolbox for the numerical evaluation of multi-scale integrals}",
    eprint = "1703.09692",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MPP-2017-42, CERN-TH-2017-063, IPPP-17-24",
    doi = "10.1016/j.cpc.2017.09.015",
    journal = "Comput. Phys. Commun.",
    volume = "222",
    pages = "313--326",
    year = "2018"
}

@article{Baikov:2019zmy,
    author = "Baikov, P. A. and Chetyrkin, K. G.",
    title = "{Transcendental structure of multiloop massless correlators and anomalous dimensions}",
    eprint = "1908.03012",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "preprint TTP19-026",
    doi = "10.1007/JHEP10(2019)190",
    journal = "JHEP",
    volume = "10",
    pages = "190",
    year = "2019"
}

@article{Baikov:2018gap,
    author = "Baikov, P. A. and Chetyrkin, K. G.",
    title = "{No-$\pi$ Theorem for Euclidean Massless Correlators}",
    eprint = "1808.00237",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.22323/1.303.0008",
    journal = "PoS",
    volume = "LL2018",
    pages = "008",
    year = "2018"
}

@article{Baikov:2018wgs,
    author = "Baikov, P. A. and Chetyrkin, K. G.",
    title = "{The structure of generic anomalous dimensions and no-$\pi$ theorem for massless propagators}",
    eprint = "1804.10088",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP06(2018)141",
    journal = "JHEP",
    volume = "06",
    pages = "141",
    year = "2018"
}

@article{Harlander:2000mg,
    author = "Harlander, Robert V.",
    title = "{Virtual corrections to g g ---\ensuremath{>} H to two loops in the heavy top limit}",
    eprint = "hep-ph/0007289",
    archivePrefix = "arXiv",
    reportNumber = "BNL-HET-00-29",
    doi = "10.1016/S0370-2693(00)01042-X",
    journal = "Phys. Lett. B",
    volume = "492",
    pages = "74--80",
    year = "2000"
}

@article{Ravindran:2004mb,
    author = "Ravindran, V. and Smith, J. and van Neerven, W. L.",
    title = "{Two-loop corrections to Higgs boson production}",
    eprint = "hep-ph/0408315",
    archivePrefix = "arXiv",
    reportNumber = "YITP-SB-04-46",
    doi = "10.1016/j.nuclphysb.2004.10.039",
    journal = "Nucl. Phys. B",
    volume = "704",
    pages = "332--348",
    year = "2005"
}

@article{Moch:2005tm,
    author = "Moch, S. and Vermaseren, J. A. M. and Vogt, A.",
    title = "{Three-loop results for quark and gluon form-factors}",
    eprint = "hep-ph/0508055",
    archivePrefix = "arXiv",
    reportNumber = "DESY-05-138, SFT-CPP-05-34, NIKHEF-05-013, DCPT-05-88, IPPP-05-44",
    doi = "10.1016/j.physletb.2005.08.067",
    journal = "Phys. Lett. B",
    volume = "625",
    pages = "245--252",
    year = "2005"
}

    
    @article{Agarwal:2021zft,
    author = "Agarwal, Bakul and von Manteuffel, Andreas and Panzer, Erik and Schabinger, Robert M.",
    title = "{Four-loop collinear anomalous dimensions in QCD and N=4 super Yang-Mills}",
    eprint = "2102.09725",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MSUHEP-21-006",
    doi = "10.1016/j.physletb.2021.136503",
    journal = "Phys. Lett. B",
    volume = "820",
    pages = "136503",
    year = "2021"
}


@article{Dixon:2017nat,
    author = "Dixon, Lance J.",
    title = "{The Principle of Maximal Transcendentality and the Four-Loop Collinear Anomalous Dimension}",
    eprint = "1712.07274",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC--PUB--17191",
    doi = "10.1007/JHEP01(2018)075",
    journal = "JHEP",
    volume = "01",
    pages = "075",
    year = "2018"
}

@article{Erdogan:2011yc,
    author = "Erdo\u{g}an, Ozan and Sterman, George",
    title = "{Gauge Theory Webs and Surfaces}",
    eprint = "1112.4564",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "YITP-SB-11-33",
    doi = "10.1103/PhysRevD.91.016003",
    journal = "Phys. Rev. D",
    volume = "91",
    number = "1",
    pages = "016003",
    year = "2015"
}

@article{Kramer:1986sg,
    author = "Kramer, G. and Lampe, B.",
    title = "{Two Jet Cross-Section in e+ e- Annihilation}",
    reportNumber = "DESY-86-103",
    doi = "10.1007/BF01679868",
    journal = "Z. Phys. C",
    volume = "34",
    pages = "497",
    year = "1987",
    note = "[Erratum: Z.Phys.C 42, 504 (1989)]"
}

@article{Matsuura:1987wt,
    author = "Matsuura, T. and van Neerven, W. L.",
    title = "{Second Order Logarithmic Corrections to the {Drell-Yan} Cross-section}",
    reportNumber = "Print-87-0792 (LEIDEN)",
    doi = "10.1007/BF01624369",
    journal = "Z. Phys. C",
    volume = "38",
    pages = "623",
    year = "1988"
}

@article{Matsuura:1988sm,
    author = "Matsuura, T. and van der Marck, S. C. and van Neerven, W. L.",
    title = "{The Calculation of the Second Order Soft and Virtual Contributions to the Drell-Yan Cross-Section}",
    reportNumber = "Print-88-0798 (LEIDEN)",
    doi = "10.1016/0550-3213(89)90620-2",
    journal = "Nucl. Phys. B",
    volume = "319",
    pages = "570--622",
    year = "1989"
}

@article{Becher:2009qa,
    author = "Becher, Thomas and Neubert, Matthias",
    title = "{On the Structure of Infrared Singularities of Gauge-Theory Amplitudes}",
    eprint = "0903.1126",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "FERMILAB-PUB-09-061-T, MZ-TH-09-05",
    doi = "10.1088/1126-6708/2009/06/081",
    journal = "JHEP",
    volume = "06",
    pages = "081",
    year = "2009",
    note = "[Erratum: JHEP 11, 024 (2013)]"
}

@article{Dokshitzer:2005ig,
    author = "Dokshitzer, Yu. L. and Marchesini, G.",
    title = "{Soft gluons at large angles in hadron collisions}",
    eprint = "hep-ph/0509078",
    archivePrefix = "arXiv",
    reportNumber = "BICOCCA-FT-05-19, LPTHE-05-23",
    doi = "10.1088/1126-6708/2006/01/007",
    journal = "JHEP",
    volume = "01",
    pages = "007",
    year = "2006"
}

@article{Dixon:2009ur,
    author = "Dixon, Lance J. and Gardi, Einan and Magnea, Lorenzo",
    title = "{On soft singularities at three loops and beyond}",
    eprint = "0910.3653",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "SLAC-PUB-13816, EDINBURGH-08-2009, DFTT-69-2009",
    doi = "10.1007/JHEP02(2010)081",
    journal = "JHEP",
    volume = "02",
    pages = "081",
    year = "2010"
}

@article{Ahrens:2012qz,
    author = "Ahrens, Valentin and Neubert, Matthias and Vernazza, Leonardo",
    title = "{Structure of Infrared Singularities of Gauge-Theory Amplitudes at Three and Four Loops}",
    eprint = "1208.4847",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MZ-TH-12-36",
    doi = "10.1007/JHEP09(2012)138",
    journal = "JHEP",
    volume = "09",
    pages = "138",
    year = "2012"
}

@article{Bern:2002tk,
    author = "Bern, Zvi and De Freitas, Abilio and Dixon, Lance J.",
    title = "{Two loop helicity amplitudes for gluon-gluon scattering in QCD and supersymmetric Yang-Mills theory}",
    eprint = "hep-ph/0201161",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-9103, UCLA-02-TEP-1",
    doi = "10.1088/1126-6708/2002/03/018",
    journal = "JHEP",
    volume = "03",
    pages = "018",
    year = "2002"
}

@article{Fadin:2021csi,
    author = "Fadin, V. S.",
    title = "{Three-Reggeon Cuts in QCD Amplitudes}",
    doi = "10.1134/S1063778820060149",
    journal = "Phys. Atom. Nucl.",
    volume = "84",
    number = "1",
    pages = "100--104",
    year = "2021"
}

@article{DelDuca:2011wkl,
    author = "Del Duca, Vittorio and Duhr, Claude and Gardi, Einan and Magnea, Lorenzo and White, Chris D.",
    title = "{An infrared approach to Reggeization}",
    eprint = "1108.5947",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "IPPP-11-47, DCPT-11-94, EDINBURGH-2011-21, DFTT-15-2011, LPN11-49",
    doi = "10.1103/PhysRevD.85.071104",
    journal = "Phys. Rev. D",
    volume = "85",
    pages = "071104",
    year = "2012"
}

@article{Kovner:2014xia,
    author = "Kovner, Alex and Lublinsky, Michael and Mulian, Yair",
    title = "{Conformal symmetry of JIMWLK Evolution at NLO}",
    eprint = "1401.0374",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP04(2014)030",
    journal = "JHEP",
    volume = "04",
    pages = "030",
    year = "2014"
}

@article{Kovner:2014lca,
    author = "Kovner, Alex and Lublinsky, Michael and Mulian, Yair",
    title = "{NLO JIMWLK evolution unabridged}",
    eprint = "1405.0418",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP08(2014)114",
    journal = "JHEP",
    volume = "08",
    pages = "114",
    year = "2014"
}

@article{Caron-Huot:2015bja,
    author = "Caron-Huot, Simon",
    title = "{Resummation of non-global logarithms and the BFKL equation}",
    eprint = "1501.03754",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP03(2018)036",
    journal = "JHEP",
    volume = "03",
    pages = "036",
    year = "2018"
}

@article{Lublinsky:2016meo,
    author = "Lublinsky, Michael and Mulian, Yair",
    title = "{High Energy QCD at NLO: from light-cone wave function to JIMWLK evolution}",
    eprint = "1610.03453",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP05(2017)097",
    journal = "JHEP",
    volume = "05",
    pages = "097",
    year = "2017"
}

@article{Schnetz:2013hqa,
    author = "Schnetz, Oliver",
    title = "{Graphical functions and single-valued multiple polylogarithms}",
    eprint = "1302.6445",
    archivePrefix = "arXiv",
    primaryClass = "math.NT",
    doi = "10.4310/CNTP.2014.v8.n4.a1",
    journal = "Commun. Num. Theor. Phys.",
    volume = "08",
    pages = "589--675",
    year = "2014"
}

@article{Brown:2004ugm,
    author = "Brown, Francis C. S.",
    title = "{Polylogarithmes multiples uniformes en une variable}",
    doi = "10.1016/j.crma.2004.02.001",
    journal = "Compt. Rend. Math.",
    volume = "338",
    number = "7",
    pages = "527--532",
    year = "2004"
}

@article{Brown:2013gia,
    author = "Brown, Francis",
    title = "{Single-valued Motivic Periods and Multiple Zeta Values}",
    eprint = "1309.5309",
    archivePrefix = "arXiv",
    primaryClass = "math.NT",
    doi = "10.1017/fms.2014.18",
    journal = "SIGMA",
    volume = "2",
    pages = "e25",
    year = "2014"
}

@article{Bassetto:1983mvz,
    author = "Bassetto, A. and Ciafaloni, M. and Marchesini, G.",
    title = "{Jet Structure and Infrared Sensitive Quantities in Perturbative QCD}",
    doi = "10.1016/0370-1573(83)90083-2",
    journal = "Phys. Rept.",
    volume = "100",
    pages = "201--272",
    year = "1983"
}

@article{Mandelstam:1965zz,
    author = "Mandelstam, S.",
    title = "{Non-Regge Terms in the Vector-Spinor Theory}",
    doi = "10.1103/PhysRev.137.B949",
    journal = "Phys. Rev.",
    volume = "137",
    pages = "B949--B954",
    year = "1965"
}

@article{Gribov:1967vfb,
    author = "Gribov, V. N.",
    title = "{A REGGEON DIAGRAM TECHNIQUE}",
    journal = "Zh. Eksp. Teor. Fiz.",
    volume = "53",
    pages = "654--672",
    year = "1967"
}

@article{Grisaru:1973wbb,
    author = "Grisaru, Marcus T. and Schnitzer, H. J. and Tsao, Hung-Sheng",
    title = "{Reggeization of elementary particles in renormalizable gauge theories - vectors and spinors}",
    doi = "10.1103/PhysRevD.8.4498",
    journal = "Phys. Rev. D",
    volume = "8",
    pages = "4498--4509",
    year = "1973"
}

@article{Grisaru:1973vw,
    author = "Grisaru, Marcus T. and Schnitzer, H. J. and Tsao, Hung-Sheng",
    title = "{Reggeization of yang-mills gauge mesons in theories with a spontaneously broken symmetry}",
    doi = "10.1103/PhysRevLett.30.811",
    journal = "Phys. Rev. Lett.",
    volume = "30",
    pages = "811--814",
    year = "1973"
}

@article{Grisaru:1973ku,
    author = "Grisaru, Marcus T. and Schnitzer, Howard J. and Tsao, Hung-Sheng",
    title = "{THE REGGEIZATION OF ELEMENTARY PARTICLES IN RENORMALIZABLE GAUGE THEORIES: SCALARS}",
    reportNumber = "Print-74-0203 (BRANDEIS)",
    doi = "10.1103/PhysRevD.9.2864",
    journal = "Phys. Rev. D",
    volume = "9",
    pages = "2864",
    year = "1974"
}

@article{Fadin:1975cb,
    author = "Fadin, Victor S. and Kuraev, E. A. and Lipatov, L. N.",
    title = "{On the Pomeranchuk Singularity in Asymptotically Free Theories}",
    doi = "10.1016/0370-2693(75)90524-9",
    journal = "Phys. Lett. B",
    volume = "60",
    pages = "50--52",
    year = "1975"
}

@book{Ioffe:2010zz,
    author = "Ioffe, Boris Lazarevich and Fadin, Victor Sergeevich and Lipatov, Lev Nikolaevich",
    title = "{Quantum chromodynamics: Perturbative and nonperturbative aspects}",
    doi = "10.1017/CBO9780511711817",
    isbn = "978-1-107-42475-3, 978-0-521-63148-8, 978-0-511-71744-4",
    publisher = "Cambridge Univ. Press",
    year = "2010"
}

@article{Caola:2021rqz,
    author = "Caola, Fabrizio and Chakraborty, Amlan and Gambuti, Giulio and von Manteuffel, Andreas and Tancredi, Lorenzo",
    title = "{Three-loop helicity amplitudes for four-quark scattering in massless QCD}",
    eprint = "2108.00055",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "MSUHEP-21-16, OUTP-21-20P",
    month = "7",
    year = "2021"
}
